BareBones: Benchmarking Zero-Shot Geometric Comprehension in VLMs

While Vision-Language Models (VLMs) demonstrate remarkable zero-shot recognition capabilities across a diverse spectrum of multimodal tasks, it yet remains an open question whether these architectures genuinely comprehend geometric structure or merely exploit RGB textures and contextual priors as statistical shortcuts. Existing evaluations fail to isolate this mechanism, conflating semantic reasoning with texture mapping and relying on imprecise annotations that inadvertently leak environmental cues. To address this gap, we introduce $\textbf{BareBones}$, a zero-shot benchmark designed to stress-test pure geometric shape comprehension. We curate pixel-level silhouettes of geometrically distinct classes across six datasets: five established segmentation sources (ImageNet-S, DIS5K, ThinObject5K, PASCAL VOC, CUB-200) and our novel flagship collection, WTP-Bench, establishing a noise-free geometric taxonomy. WTP-Bench is an extreme, fine-grained visual puzzle that forces models to identify inter-class geometric concepts from boundary contours alone. Our evaluation of 26 state-of-the-art proprietary and open-weight VLMs (eg. GPT-4.1, Gemini, Claude Sonnet 4.5, LLaVA) reveals a consistent, severe performance collapse under RGB deprivation, a phenomenon we term the $\textit{Texture Bias Cliff}$. By documenting universal structural blindspots, BareBones establishes a rigorous yardstick for genuine geometric grounding. Project Page: https://eternal-f1ame.github.io/WTP-Bench/

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related_work}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/scatter_performance.pdf}
\caption{\textbf{Texture Bias Cliff Scatter Plot.} True geometric understanding demands high accuracy regardless of RGB texture (ideal models lie along the dashed line). Instead, all models cluster at the bottom right, suggesting over-reliance on texture over global shape.}
\label{fig:scatter_performance}
\end{figure}



\noindent \textbf{Zero-Shot Visual Recognition and Generalist VLMs:}
The transition from highly specialized, task-specific architectures to zero-shot, general-purpose Vision-Language Models (VLMs) has been driven by massive-scale pretraining on vast corpora of interleaved image-text datasets. Foundation models such as CLIP \cite{radford2021learning} and ALIGN \cite{jia2021scaling} pioneered the contrastive alignment of text-image pairs, establishing highly robust representations that easily transfer to novel distributions. More recently, autoregressive architectures incorporating explicit language decoders, such as LLaVA \cite{liu2024llava}, GPT-4.1 \cite{openai2023gpt4}, Gemini \cite{team2023gemini}, and the rapidly evolving Qwen-VL series \cite{bai2023qwen}, integrate immensely powerful Large Language Models (LLMs) with advanced visual encoders (predominantly Vision Transformers, or ViTs). These generalist models excel at a variety of complex multimodal tasks ranging from detailed image captioning and visual question answering (VQA) to profound logical reasoning and code generation. Their remarkable success has prompted critical investigations into the \textit{source} of their emergent capabilities: do these models genuinely possess a structural, conceptual understanding of the physical world, or are they merely sophisticated aggregators of superficial, high-frequency statistical features mapped perfectly to extensive textual priors? Our work directly probes this generalization capacity by surgically severing the most common heuristic models exploit-superficial mapping cues like color and texture.

\input{tables/model_identifiers}


\noindent \textbf{VLM Benchmarking and the Geometric Gap:}
To quantify the rapid evolution of multimodal capabilities, modern benchmarking suites have proliferated dramatically, aiming to test the limits of VLMs across exceedingly diverse cognitive dimensions. Benchmarks like MMVP \cite{tong2024eyes} probe fundamental perceptual vulnerabilities, MathVista \cite{lu2023mathvista} demands rigorous visual mathematical reasoning, and specialized suites like SEED-Bench \cite{li2023seed} evaluate fine-grained categorical knowledge. However, despite this aggressive expansion of multimodal evaluations, a critical gap remains: prevailing benchmarks overwhelmingly test complex semantic correlation that is intrinsically intertwined with local texture, color gradients, and heavy background priors. A model evaluating an image from classic datasets like COCO or general ImageNet can bypass structural geometry entirely by locking onto the distinctive spotted texture of a cheetah or the vivid blue of an ocean background. Precise geometric grounding, particularly concerning the exact tracing of fine-grained boundaries lacking distinct internal shading, is frequently obfuscated. The BareBones benchmark was explicitly constructed to fill this glaring void. By strictly eliminating textures, lighting, and contextual cues through absolute bi-level thresholding across diverse established taxonomies, BareBones enforces a rigorous evaluation exclusively focused on pure, unassisted structural and silhouette-based reasoning.




\noindent \textbf{Texture Bias vs. Shape Bias in Machine Vision:}
The debate concerning whether Convolutional Neural Networks (CNNs) and contemporary Vision Transformers (ViTs) rely predominantly on global \textit{shape} or local \textit{texture} is extensively documented within traditional computer vision literature. Foundational psychophysical and empirical studies \cite{geirhos2018imagenettrained} famously revealed that classic ImageNet-trained CNNs exhibit a severe, almost pathological texture bias. These architectures consistently classify images correctly based purely on local surface patterns (\eg identifying the crinkled texture of elephant skin) while failing spectacularly when an object's distinct shape is filled with conflicting textures (e.g., a cat silhouette mapped with elephant skin). While subsequent research has heavily explored augmenting training data with aggressive stylization, varying image frequencies, and edge-map distillations to forcefully encourage shape bias \cite{hermann2020origins, nasekov2023investigating}, this fundamental debate has yet to be comprehensively analyzed at the immense scale of multimodal Large Language Models across extreme, fine-grained taxonomies. Furthermore, it is unknown whether the inclusion of billions of parameters in the LLM backbone can compensate for, or perhaps even exacerbate, the visual encoder's innate texture dependence. BareBones extends this cue-conflict evaluation paradigm---originally applied to CNNs via stylized images---directly into the generative VLM era, quantifying the magnitude of the ``Texture Bias Cliff'' in contemporary open-weight and frontier architectures under a more severe condition: complete RGB deprivation rather than texture-style transfer.

==> tables/evaluation_datasets.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Evaluation Datasets.} High-fidelity segmentation datasets utilized to benchmark pure structural reasoning.}
\label{tab:datasets}
\begin{tabularx}{\linewidth}{|l|r|Y|}
\toprule
\rowcolor{shadecolor} \textbf{Dataset} & \textbf{Targets} & \textbf{Geometric Focus / Challenge} \\
\midrule
ImageNet-S \cite{gao2022large} & 100 & Base geometric identities and distinctive structural outlines. \\
DIS5K \cite{qin2022highly} & 125 & Highly precise segmentation; complex boundaries, fine appendages, and negative spaces. \\
ThinObject5K \cite{liew2021deep} & 193 & Tracking continuous, narrow geometries lacking large contiguous texture regions. \\
PASCAL VOC \cite{everingham2010pascal} & 20 & Articulated objects ensuring diversity in pose and geometry-obfuscating occlusions. \\
CUB-200 \cite{wah2011caltech} & 200 & Fine-grained inter-class discrimination differentiating highly similar core avian body shapes through minute beak, tail, and crest geometry. \\
WTP-Bench (Ours) & 1,160 & Flagship visual puzzle; extreme fine-grained associative geometry spanning 8 generational taxonomies. \\
\bottomrule
\end{tabularx}
\end{table}

==> tables/hallucination_bias.tex <==
\begin{table}[t]
\centering
\small
\captionof{table}{\textbf{Hallucination Bias Distribution.} Frequency of incorrect predictions by the 16 open-weight models mapped to generational taxonomies, revealing a massive, statistically disproportionate bias towards Generation~1 textual priors when visual signals fail.}
\label{tab:gen1_bias}
\begin{tabularx}{\linewidth}{|Y|rr | r|}
\toprule
\rowcolor{shadecolor} & \multicolumn{2}{c|}{\textbf{Open-Weight Silhouette Errors}} & \\
\cmidrule(lr){2-3}
\rowcolor{shadecolor}\textbf{Generation} & \textbf{Wrong Guesses} & \textbf{\% of Errors} & \textbf{Dataset \%} \\
\midrule
1 & 13,959 & \textbf{79.2\%} & 19.6\% \\
2 & 1,156 & 6.6\% & 9.6\% \\
3 & 613 & 3.5\% & 14.2\% \\
4 & 868 & 4.9\% & 11.2\% \\
5 & 371 & 2.1\% & 15.9\% \\
6 & 372 & 2.1\% & 9.4\% \\
7 & 174 & 1.0\% & 9.0\% \\
8 & 108 & 0.6\% & 11.1\% \\
\bottomrule
\end{tabularx}
\end{table}

==> tables/universally_hard_wtp_gen.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{minipage}[t]{0.44\linewidth}
\centering
\begin{tabular}{|l|c|}
\toprule
\rowcolor{shadecolor} \textbf{Class} & \textbf{HQ Acc (\%)} \\
\midrule
\multicolumn{2}{|c|}{\cellcolor{LGray2}\textbf{WTP-Bench}} \\
\midrule
Eternatus (Eternamax) & 54.2 \\
Dugtrio (Alolan) & 62.1 \\
Slowbro (Galarian) & 71.6 \\
\midrule
\multicolumn{2}{|c|}{\cellcolor{LGray2}\textbf{ImageNet-S}} \\
\midrule
Green Mamba & 48.3 \\
Diamondback & 55.1 \\
\midrule
\multicolumn{2}{|c|}{\cellcolor{LGray2}\textbf{CUB-200}} \\
\midrule
Blue Jay & 52.8 \\
Indigo Bunting & 33.3 \\
\midrule
\multicolumn{2}{|c|}{\cellcolor{LGray2}\textbf{DIS5K}} \\
\midrule
Fire Extinguisher & 43.8 \\
Monitor & 51.2 \\
\midrule
\multicolumn{2}{|c|}{\cellcolor{LGray2}\textbf{PASCAL VOC \& ThinObject5K}} \\
\midrule
Potted Plant & 37.4 \\
Boots & 56.2 \\
\bottomrule
\end{tabular}
\caption{\textbf{Universally Hard Targets.} Classes achieving $0.0\%$ exact-match accuracy across all 26 models in silhouette format. High HQ accuracy confirms these are not ambiguous classes but genuine geometric blindspots.}
\label{tab:universally_hard}
\end{minipage}
\hfill
\begin{minipage}[t]{0.54\linewidth}
\centering
\begin{tabular}{|l|c|c||c|c|}
\toprule
\rowcolor{shadecolor} & \multicolumn{2}{c||}{\textbf{Generation 1}} & \multicolumn{2}{c|}{\textbf{Generation 8}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\rowcolor{shadecolor} \textbf{Model} & \textbf{HQ (\%)} & \textbf{Sil (\%)} & \textbf{HQ (\%)} & \textbf{Sil (\%)} \\
\midrule
\multicolumn{5}{|c|}{\cellcolor{LGray2}\textbf{Proprietary Models}} \\
\midrule
GPT-4.1          & 85.4 & 58.2 & 71.2 & 38.5 \\
Gemini 2.5 Pro   & 81.3 & 29.1 & 73.4 & 15.2 \\
Claude Sonnet 4.5 & 74.2 & 33.6 & 55.1 & 18.4 \\
\midrule
\multicolumn{5}{|c|}{\cellcolor{LGray2}\textbf{Open-Weight Models}} \\
\midrule
LLaVA 1.5 7B   & 18.5 & 4.2 & 5.1 & 0.2 \\
LLaVA 1.5 13B  & 2.1  & 1.2 & 0.3 & 0.0 \\
Ovis2.5 9B     & 22.1 & 3.8 & 4.0 & 0.0 \\
\bottomrule
\end{tabular}
\caption{\textbf{Pre-training Memorization Bias.} Exact-match accuracy on Generation~1 vs.\ Generation~8 targets. The consistent HQ--silhouette regression across both generations confirms models rely on pretraining priors, not geometric reasoning.}
\label{tab:wtp_generations}
\end{minipage}
\end{table*}

